Stopping Is Not the Limit: Understanding and Eliciting Agent Capability in Long-Horizon Vulnerability Exploitation

Vulnerability exploitation tests whether language model agents can develop working exploits from known software flaws. Sequential test-time scaling can improve exploitation performance, but larger budgets do not ensure sustained exploration: agents often stop with budget remaining. Yet what happens when execution continues beyond stopping remains underexplored. We investigate this gap on ExploitBench using DeepSeek-V4-Flash-0731 and MiMo-V2.6-Pro. We find additional verified gains after the first stop response, but gains diminish over longer execution. We identify two patterns associated with less productive continuation: an increasing proportion of stop responses within the same context and earlier stopping associated with summaries retaining impossibility judgments about unachieved capabilities. To test whether context management can elicit further capability, we propose SCoRe, which compacts context at stop bursts and marks these judgments as unproven. SCoRe improves verified capability over summary-based continuation and other evaluated context-management baselines. With SCoRe, MiMo reaches a capability coverage score of 67.0% at 2,000 turns, exceeding both 32.4% under the original stopping policy and the 58.6% computed for GPT-5.5 from ExploitBench's 300-turn reference results on the same tasks. These findings show that stopping need not mark an agent's exploitation limit, and that continued execution with context management can elicit substantial further capability.

==> figures/score-style.tex <==
% SCoRe overview. Input directly in figure*: native size 16 x 8 cm.
% Requires LuaLaTeX or XeLaTeX, fontspec, Font Awesome 5, TikZ (arrows.meta, calc),
% and commands/paper-style.tex. All figure-specific definitions are local.

% Design language and hierarchy:
% 1. Trajectories: neutral lanes and tool-call response tiles, white context tiles,
%    and red octagonal STOP signs for stop responses.
% 2. New summary: one quiet gray document surface on the left, with six rows.
% 3. Peer methods: identical white panels and semibold titles, with balanced
%    red stop and blue relabeling accents on outlines and icons.
%    No flags or event-level judgment classification are shown.
% 4. Examples: a standalone rectangular example and a separate section-6 inset.
%    Titles sit above their contents; quotes lead over smaller annotations.
%    There is no divider or transformation path between the two examples.
%    A red cross and green check distinguish avoided and preferred wording;
%    their shapes preserve the distinction independently of color.
% All geometry is square, flat, and shadow-free. Every structural stroke is
% 0.4pt; hierarchy comes from spacing, type weight, surfaces, and contrast.
% Arrows carry the complete context into and out of one summary call.
% Dashed, arrow-free guides indicate magnification, not a processing step.
\newfontfamily\ScoreSans{Inter-Regular.otf}[
  Ligatures=TeX,BoldFont={Inter-SemiBold.otf}]
% Type and icon roles are specified in actual printed points.
\newcommand{\ScoreBodyFont}{\ScoreSans\fontsize{8.5}{10.5}\selectfont}
\newcommand{\ScoreQuoteFont}{\ScoreSans\fontsize{9.5}{12}\selectfont}
\newcommand{\ScoreMethodFont}{\ScoreSans\bfseries\fontsize{9.5}{11.5}\selectfont}
\newcommand{\ScoreSectionFont}{\ScoreSans\bfseries\fontsize{9}{11}\selectfont}
\newcommand{\ScoreMetaFont}{\ScoreSans\fontsize{7.5}{9}\selectfont}
\newcommand{\ScoreAgentFont}{\fontsize{9}{9}\selectfont}
\newcommand{\ScoreCellIconFont}{\fontsize{7.5}{7.5}\selectfont}
\newcommand{\ScoreStopFont}{\ScoreSans\bfseries\fontsize{4}{4}\selectfont}
\newcommand{\ScoreTitleIconFont}{\fontsize{8.5}{8.5}\selectfont}
\colorlet{ScoreBandFill}{CapybaraFindingBackground}
\colorlet{ScoreNeutralRule}{CapybaraFindingBorder!75!white}
\colorlet{ScoreScopeRule}{CapybaraLine}
\colorlet{ScoreScopeFill}{CapybaraFindingBackground}
% Component/control colors, independent of the paper's model-series palette.
% Matched OKLCH lightness/chroma: accents L=.57, C=.18; pale fills L=.96, C=.018.
% Stop hue=25 degrees, relabeling hue=260 degrees; rounded to 8-bit sRGB.
\colorlet{ScoreToolFill}{CapybaraFindingBackground}
\definecolor{ScoreStopAccent}{HTML}{CC3D3D}
\definecolor{ScoreStopPale}{HTML}{FEEDEC}
\definecolor{ScoreRelabelAccent}{HTML}{3072DF}
\definecolor{ScoreRelabelPale}{HTML}{EBF2FE}
\colorlet{ScoreAvoidedWording}{ScoreStopAccent}
\definecolor{ScorePreferredWording}{HTML}{25844C}

% Native design system: physical coordinates in cm, strokes in pt.
% The artwork is drawn at final size. There is no fitting or scale transform.
% The only edge inset is half a stroke, keeping boundary rules on the page.
\def\ScoreWidth{16}
\def\ScoreAspectRatio{2}
\pgfmathsetmacro{\ScoreHeight}{\ScoreWidth/\ScoreAspectRatio}
\def\ScoreBorder{0.4pt}
\def\ScoreTextHeight{1.5ex}
\def\ScoreTextDepth{0.4ex}
\def\ScoreArrowLength{1.4mm}
\def\ScoreArrowWidth{1.0mm}
\def\ScorePadding{0.20}
\def\ScorePanelPadding{0.15}
% The shared title band leaves about .18 cm above and below the title ink,
% matching the .15--.20 cm padding used around the neighboring contents.
\def\ScoreHeaderHeight{0.60}
\def\ScoreCellSize{0.50}
\let\ScoreCellGap\ScorePanelPadding
\pgfmathsetmacro{\ScorePitch}{\ScoreCellSize+\ScoreCellGap}
\def\ScoreStopRadius{0.195}
\pgfmathsetmacro{\ScoreStopCorner}{\ScoreStopRadius*tan(22.5)}
\let\ScoreLegendGap\ScorePanelPadding
\def\ScoreLegendEntryGap{0.55}
\def\ScoreAgentInset{0.35}
\let\ScoreTitleIconGap\ScorePanelPadding
\def\ScoreTitleIconSlot{0.40}
\def\ScoreContextInset{0.80}
\def\ScoreTaskWidth{1.15}
\let\ScoreWindowPadding\ScorePanelPadding
\def\ScorePrefixCount{3}
\def\ScoreWindowCount{14}
\let\ScoreConditionInset\ScorePanelPadding
\let\ScoreHistoryGap\ScorePanelPadding
\def\ScoreHistoryTick{0.10}
\def\ScoreOutputWidth{4.40}
\def\ScoreOutputGap{1.20}
\let\ScoreNumberInset\ScorePadding
\def\ScoreFieldInset{0.45}

% Two-column middle layout: one output document and two explanatory insets.
\def\ScoreSummaryHeaderHeight{0.65}
\def\ScoreMiddleTop{5.65}
\def\ScoreMiddleBottom{1.35}
\def\ScoreAnnotationGap{0.15}
% Edge-anchored trajectories keep their original physical geometry.
\pgfmathsetmacro{\ScoreStrokeInset}{(\ScoreBorder)/2/1cm}
\let\ScoreLeft\ScoreStrokeInset
\pgfmathsetmacro{\ScoreRight}{\ScoreWidth-\ScoreStrokeInset}
\pgfmathsetmacro{\ScoreTop}{\ScoreHeight-\ScoreStrokeInset}
\pgfmathsetmacro{\ScoreBandHalfHeight}{\ScoreCellSize/2+\ScoreWindowPadding}
\pgfmathsetmacro{\ScoreUpperY}{\ScoreTop-\ScoreHeaderHeight-\ScoreBandHalfHeight}
\let\ScoreLowerY\ScoreBandHalfHeight
\pgfmathsetmacro{\ScoreWindowBodyTop}{\ScoreUpperY+\ScoreBandHalfHeight}
\pgfmathsetmacro{\ScoreWindowBottom}{\ScoreUpperY-\ScoreBandHalfHeight}
\pgfmathsetmacro{\ScoreWindowTitleY}{\ScoreWindowBodyTop+\ScoreHeaderHeight/2}

% Horizontal frame widths and the shared pitch of the two trajectories.
\pgfmathsetmacro{\ScoreAgentX}{\ScoreLeft+\ScoreAgentInset}
\pgfmathsetmacro{\ScoreContextLeft}{\ScoreLeft+\ScoreContextInset}
\pgfmathtruncatemacro{\ScoreEventCount}{\ScorePrefixCount+\ScoreWindowCount}
% Anchor the fixed-pitch event row to the right edge; the summary field takes
% the remaining context width, so spacing never stretches to fill the lane.
\pgfmathsetmacro{\ScoreContextRight}{\ScoreRight-\ScoreWindowPadding-\ScoreEventCount*\ScorePitch}
\pgfmathsetmacro{\ScoreTaskRight}{\ScoreContextLeft+\ScoreTaskWidth}
\pgfmathsetmacro{\ScoreTaskCenter}{(\ScoreContextLeft+\ScoreTaskRight)/2}
\pgfmathsetmacro{\ScoreSummaryInputLeft}{\ScoreTaskRight+\ScoreCellGap}
\pgfmathsetmacro{\ScoreSummaryInputCenter}{(\ScoreSummaryInputLeft+\ScoreContextRight)/2}
\pgfmathsetmacro{\ScoreEventsLeft}{\ScoreContextRight+\ScoreCellGap}
\pgfmathsetmacro{\ScoreEventsRight}{\ScoreEventsLeft+\ScoreEventCount*\ScorePitch-\ScoreCellGap}
\pgfmathsetmacro{\ScoreUpperBandRight}{\ScoreEventsRight+\ScoreWindowPadding}
\pgfmathsetmacro{\ScoreWindowEventsLeft}{\ScoreEventsLeft+\ScorePrefixCount*\ScorePitch}
\pgfmathsetmacro{\ScoreWindowLeft}{\ScoreWindowEventsLeft-\ScoreWindowPadding}
\pgfmathsetmacro{\ScoreHistoryY}{\ScoreWindowBottom-\ScoreHistoryGap}
\pgfmathsetmacro{\ScoreOutputRight}{\ScoreLeft+\ScoreOutputWidth}
% Align the summary drop with the task's left edge, keeping its label inside
% the left-hand column instead of extending across the inter-column gap.
\let\ScoreSummarizeX\ScoreContextLeft
\pgfmathsetmacro{\ScoreSummarizeY}{(\ScoreHistoryY+\ScoreMiddleTop)/2}
\pgfmathsetmacro{\ScoreMiddleTitleY}{\ScoreMiddleTop-\ScoreSummaryHeaderHeight/2}
\pgfmathsetmacro{\ScoreSummaryLeft}{\ScoreLeft+\ScorePadding}
\pgfmathsetmacro{\ScoreSummaryRight}{\ScoreOutputRight-\ScorePadding}
\pgfmathsetmacro{\ScoreSummaryTop}{\ScoreMiddleTop-\ScoreSummaryHeaderHeight}
\pgfmathsetmacro{\ScoreSummaryBottom}{\ScoreMiddleBottom+\ScorePadding}
\pgfmathsetmacro{\ScoreFieldHeight}{(\ScoreSummaryTop-\ScoreSummaryBottom)/6}
\pgfmathsetmacro{\ScoreConclusionTop}{\ScoreSummaryBottom+\ScoreFieldHeight}
\pgfmathsetmacro{\ScoreExamplesLeft}{\ScoreOutputRight+\ScoreOutputGap}
\pgfmathsetmacro{\ScoreCardLeft}{\ScoreExamplesLeft+\ScorePadding}
\pgfmathsetmacro{\ScoreCardRight}{\ScoreRight-\ScorePadding}
\pgfmathsetmacro{\ScoreCardTextLeft}{\ScoreCardLeft+\ScorePadding}
\pgfmathsetmacro{\ScoreCardTextWidth}{\ScoreCardRight-\ScoreCardLeft-2*\ScorePadding}

% Content determines card heights. Both quotations wrap naturally in the same
% paragraph width; annotations use the smaller secondary typography.
% The original quote is from figure_Capybara/tables/rq2_summary_examples.tex,
% ASAN row (crbug-339064932, seed 1, segment 1). It is a summary excerpt,
% independent of the schematic response sequence above.
% The rewrite follows the summary prompt; annotations use the paper's terms.
\newcommand{\ScoreJudgmentTitle}{Capability-level impossibility judgment}
\newcommand{\ScoreConclusionTitle}{Unproven conclusions}
\newcommand{\ScoreConclusionDescription}{Tentative conclusions limited to the approaches tried}
\newcommand{\ScoreJudgmentQuote}{\textquotedblleft the asan capability is \textbf{unreachable}.\textquotedblright}
\newcommand{\ScoreRewriteQuote}{\textquotedblleft I have \textbf{not yet found a way} to achieve asan through the approaches I attempted.\textquotedblright}
% Attach each wording marker to its quotation without an isolated line break.
\newcommand{\ScoreWordingMarker}[2]{%
  \nobreak\hspace{\ScoreAnnotationGap cm}%
  \mbox{\textcolor{#1}{{\ScoreTitleIconFont #2}}}%
}
\newsavebox{\ScoreJudgmentMeasure}
\newsavebox{\ScoreRewriteMeasure}
\sbox{\ScoreJudgmentMeasure}{\parbox[t]{\ScoreCardTextWidth cm}{%
  \raggedright\parindent=0pt\parskip=0pt\color{CapybaraInk}%
  {\ScoreQuoteFont\ScoreJudgmentQuote\ScoreWordingMarker{ScoreAvoidedWording}{\faTimes}\par}%
  \vspace{\ScoreAnnotationGap cm}%
  {\ScoreMetaFont\color{CapybaraMuted}\ScoreJudgmentTitle\par}%
}}
\sbox{\ScoreRewriteMeasure}{\parbox[t]{\ScoreCardTextWidth cm}{%
  \raggedright\parindent=0pt\parskip=0pt\color{CapybaraInk}%
  {\ScoreSectionFont 6\enspace\ScoreConclusionTitle\par}%
  \vspace{\ScoreAnnotationGap cm}%
  {\ScoreQuoteFont\ScoreRewriteQuote\ScoreWordingMarker{ScorePreferredWording}{\faCheck}\par}%
  \vspace{\ScoreAnnotationGap cm}%
  {\ScoreMetaFont\color{CapybaraMuted}\ScoreConclusionDescription\par}%
}}
\pgfmathsetmacro{\ScoreJudgmentHeight}{(\the\ht\ScoreJudgmentMeasure+\the\dp\ScoreJudgmentMeasure)/1cm}
\pgfmathsetmacro{\ScoreRewriteHeight}{(\the\ht\ScoreRewriteMeasure+\the\dp\ScoreRewriteMeasure)/1cm}
% Both outer panels share their top and bottom edges. The header includes its
% own vertical padding; anchor each measured card to the adjacent panel edge
% and leave the remaining space between the cards.
\let\ScoreExamplesTop\ScoreMiddleTop
\let\ScoreExamplesBottom\ScoreMiddleBottom
\pgfmathsetmacro{\ScoreZoomBottom}{\ScoreExamplesBottom+\ScorePadding}
\pgfmathsetmacro{\ScoreZoomTop}{\ScoreZoomBottom+\ScoreRewriteHeight+2*\ScorePadding}
\pgfmathsetmacro{\ScoreJudgmentTop}{\ScoreExamplesTop-\ScoreHeaderHeight}
\pgfmathsetmacro{\ScoreJudgmentBottom}{\ScoreJudgmentTop-\ScoreJudgmentHeight-2*\ScorePadding}
\pgfmathsetmacro{\ScoreMethodTitleY}{\ScoreExamplesTop-\ScoreHeaderHeight/2}

% Right-align the legend on the bottom row and let the resumed lane extend
% up to a fixed gap before it. The measured labels determine both boundaries.
\newcommand{\ScoreToolLegend}{Tool-call response}
\newcommand{\ScoreStopLegend}{Stop response (no tool call)}
\newsavebox{\ScoreToolLegendMeasure}
\newsavebox{\ScoreStopLegendMeasure}
\sbox{\ScoreToolLegendMeasure}{\ScoreMetaFont\ScoreToolLegend}
\sbox{\ScoreStopLegendMeasure}{\ScoreMetaFont\ScoreStopLegend}
\pgfmathsetmacro{\ScoreToolLegendWidth}{\ScoreCellSize+\ScoreLegendGap+\the\wd\ScoreToolLegendMeasure/1cm}
\pgfmathsetmacro{\ScoreStopLegendWidth}{\ScoreCellSize+\ScoreLegendGap+\the\wd\ScoreStopLegendMeasure/1cm}
\pgfmathsetmacro{\ScoreLegendWidth}{\ScoreToolLegendWidth+\ScoreLegendEntryGap+\ScoreStopLegendWidth}
\pgfmathsetmacro{\ScoreLegendLeft}{\ScoreRight-\ScoreLegendWidth}
\pgfmathsetmacro{\ScoreLowerBandRight}{\ScoreLegendLeft-\ScoreLegendEntryGap}
\pgfmathsetmacro{\ScoreLegendToolX}{\ScoreLegendLeft+\ScoreCellSize/2}
\pgfmathsetmacro{\ScoreLegendStopX}{\ScoreLegendToolX+\ScoreToolLegendWidth+\ScoreLegendEntryGap}

\tikzset{
  score figure/.style={every node/.style={font=\ScoreBodyFont,text=CapybaraInk,
      inner sep=0pt,outer sep=0pt},sharp corners,line cap=butt,line join=miter},
  score label/.style={text height=\ScoreTextHeight,text depth=\ScoreTextDepth},
  score border/.style={draw=ScoreNeutralRule,line width=\ScoreBorder},
  score scope/.style={draw=ScoreScopeRule,line width=\ScoreBorder},
  score context/.style={score border,fill=white},
  score event/.style={score border,fill=white},
  score tool/.style={fill=ScoreToolFill},
  score stop/.style={draw=ScoreStopAccent,fill=ScoreStopPale},
  score connector/.style={draw=CapybaraMuted,line width=\ScoreBorder},
  score arrow/.style={-{Stealth[length=\ScoreArrowLength,width=\ScoreArrowWidth]}},
  score flow/.style={score connector,score arrow},
  score zoom source/.style={draw=ScoreRelabelAccent,line width=\ScoreBorder},
  score zoom/.style={score zoom source,dash pattern=on 2pt off 2pt},
  score method border/.style={draw=#1,line width=\ScoreBorder},
  score method frame/.style={score method border=#1,fill=white}
}

% Drawing primitives: response icons shared by cells and the legend, panels,
% and summary examples. Response cells share one neutral geometry.
\newcommand{\ScoreAgent}[2]{%
  \node[font=\ScoreAgentFont] at (#1,#2) {\faRobot};
}
\newcommand{\ScoreCell}[4]{%
  \path[score event,#4] (#1,{#2-\ScoreCellSize/2})
    rectangle ({#1+\ScoreCellSize},{#2+\ScoreCellSize/2});
  #3{#1+\ScoreCellSize/2}{#2}%
}
\newcommand{\ScoreToolIcon}[2]{%
  \node[text=CapybaraMuted,font=\ScoreCellIconFont] at (#1,#2) {\faWrench};
}
\newcommand{\ScoreStopIcon}[2]{%
  \path[fill=ScoreStopAccent]
    ({#1-\ScoreStopCorner},{#2+\ScoreStopRadius})
    --({#1+\ScoreStopCorner},{#2+\ScoreStopRadius})
    --({#1+\ScoreStopRadius},{#2+\ScoreStopCorner})
    --({#1+\ScoreStopRadius},{#2-\ScoreStopCorner})
    --({#1+\ScoreStopCorner},{#2-\ScoreStopRadius})
    --({#1-\ScoreStopCorner},{#2-\ScoreStopRadius})
    --({#1-\ScoreStopRadius},{#2-\ScoreStopCorner})
    --({#1-\ScoreStopRadius},{#2+\ScoreStopCorner})--cycle;
  \node[text=white,font=\ScoreStopFont] at (#1,#2) {STOP};
}
\newcommand{\ScoreTool}[2]{\ScoreCell{#1}{#2}{\ScoreToolIcon}{score tool}}
\newcommand{\ScoreStop}[2]{\ScoreCell{#1}{#2}{\ScoreStopIcon}{score stop}}
\newcommand{\ScoreLegendEntry}[3]{%
  #2{#1}{\ScoreLowerY}%
  \node[score label,anchor=west,font=\ScoreMetaFont]
    at ({#1+\ScoreCellSize/2+\ScoreLegendGap},\ScoreLowerY) {#3};
}
\newcommand{\ScoreEllipsis}[2]{%
  \node[text=CapybaraMuted] at ({#1+\ScoreCellSize/2},#2) {$\cdots$};
}
\newcommand{\ScoreSequence}[3]{%
  \foreach \eventindex/\eventkind in #3 {
    \csname Score\eventkind\endcsname{#1+\eventindex*\ScorePitch}{#2}
  }
}
\newcommand{\ScoreTrajectory}[3]{%
  \path[fill=ScoreBandFill] (\ScoreLeft,{#1-\ScoreBandHalfHeight})
    rectangle (#3,{#1+\ScoreBandHalfHeight});
  \ScoreAgent{\ScoreAgentX}{#1}
  \path[score context] (\ScoreContextLeft,{#1-\ScoreCellSize/2})
    rectangle (\ScoreTaskRight,{#1+\ScoreCellSize/2});
  \node[score label,anchor=center] at (\ScoreTaskCenter,#1) {Task};
  \path[score context] (\ScoreSummaryInputLeft,{#1-\ScoreCellSize/2})
    rectangle (\ScoreContextRight,{#1+\ScoreCellSize/2});
  \node[score label,anchor=center] at (\ScoreSummaryInputCenter,#1) {#2};
}
% Title icons share a fixed slot, and their ink center follows the cap-height
% center of the adjacent title. The complete row is centered in its band.
\newcommand{\ScoreTitleIcon}[3]{%
  \makebox[\ScoreTitleIconSlot cm][c]{%
    \raisebox{\dimexpr(#1-\height+\depth)/2\relax}{%
      \textcolor{#2}{{\ScoreTitleIconFont #3}}}}%
  \hspace{\ScoreTitleIconGap cm}%
}
\newcommand{\ScoreHeading}[5]{%
  \node[anchor=base west,font=#3,yshift={\dimexpr-#4/2\relax}]
    at (#1,#2) {#5};
}
\newcommand{\ScoreMethodTitle}[5]{%
  \ScoreHeading{#1}{#2}{\ScoreMethodFont}{\ht\ScoreMethodCap}
    {\ScoreTitleIcon{\ht\ScoreMethodCap}{#5}{#4}#3}%
}
\newcommand{\ScoreMethod}[7]{%
  \path[score method frame=#7] (#1,#2) rectangle (#3,{#4+\ScoreHeaderHeight});
  \ScoreMethodTitle{#1+\ScorePanelPadding}{#4+\ScoreHeaderHeight/2}{#5}{#6}{#7}%
}

% Measure title cap heights outside TikZ so icon/text alignment is independent
% of each glyph's font bounding box or descender depth.
\newsavebox{\ScoreSectionCap}
\newsavebox{\ScoreMethodCap}
\sbox{\ScoreSectionCap}{\ScoreSectionFont H}
\sbox{\ScoreMethodCap}{\ScoreMethodFont H}

% Schematic sequences, not counts used to evaluate the real W=20 window.
% Stop and wrench cells denote stop and tool-call responses, respectively.
% Ellipses abbreviate the full detector window.
\def\ScorePrefixSequence{0/Tool,1/Tool,2/Ellipsis}
\def\ScoreWindowSequence{0/Tool,1/Tool,2/Stop,3/Tool,4/Stop,5/Ellipsis,
  6/Tool,7/Tool,8/Stop,9/Tool,10/Tool,11/Tool,12/Tool,13/Stop}


% The trajectory bands are shared verbatim by the paper and layout studies.
\newcommand{\ScoreUpperTrajectory}{%
\ScoreTrajectory{\ScoreUpperY}{Prior summary}{\ScoreUpperBandRight}
\ScoreSequence{\ScoreEventsLeft}{\ScoreUpperY}{\ScorePrefixSequence}
\ScoreMethod{\ScoreWindowLeft}{\ScoreWindowBottom}{\ScoreUpperBandRight}{\ScoreWindowBodyTop}
  {Stop-aware compaction}{\faBolt}{ScoreStopAccent}
\node[score label,anchor=east,font=\ScoreMetaFont]
  at ({\ScoreUpperBandRight-\ScoreConditionInset},\ScoreWindowTitleY) {stop-response fraction $\geq\rho$};
\ScoreSequence{\ScoreWindowEventsLeft}{\ScoreUpperY}{\ScoreWindowSequence}
}
\newcommand{\ScoreLowerTrajectory}{%
  \ScoreTrajectory{\ScoreLowerY}{New summary}{\ScoreLowerBandRight}
  \ScoreEllipsis{\ScoreEventsLeft}{\ScoreLowerY}
  \ScoreLegendEntry{\ScoreLegendToolX}{\ScoreToolIcon}{\ScoreToolLegend}
  \ScoreLegendEntry{\ScoreLegendStopX}{\ScoreStopIcon}{\ScoreStopLegend}
}

